Optimizing City-Wide White-Fi Networks in TV White Spaces

White-Fi refers to WiFi deployed in the TV white spaces. Unlike its ISM band counterparts, White-Fi must obey requirements that protect TV reception. As a result, optimization of citywide White-Fi networks faces the challenges of heterogeneous channel availability and link quality, over location. The former is because, at any location, channels in use by TV networks are not available for use by White-Fi. The latter is because the link quality achievable at a White-Fi receiver is determined by not only its link gain to its transmitter but also by its link gains to TV transmitters and its transmitter's link gains to TV receivers. In this work, we model the medium access control (MAC) throughput of a White-Fi network. We propose heuristic algorithms to optimize the throughput, given the described heterogeneity. The algorithms assign power, access probability, and channels to nodes in the network, under the constraint that reception at TV receivers is not compromised. We evaluate the efficacy of our approach over example city-wide White-Fi networks deployed over Denver and Columbus (respectively, low and high channel availability) in the USA, and compare with assignments cognizant of heterogeneity to a lesser degree, for example, akin to FCC regulations.

==> Discussion.tex <==
\section{Discussion}
\label{sec:discussion}
The IEEE $802.11$af standard~\cite{TVstandard} proposes an architecture that enables operation of secondary networks in compliance with a multitude of regulatory mechanisms designed to protect the TV network. Figure~\ref{fig:80211afArch} shows the essential components of the architecture and how the architecture can be leveraged to execute the proposed algorithms.
\begin{figure}
\centering
\includegraphics[scale=0.5]{Figures/architecture_ver4.pdf}
\caption{\small Architecture, similar to the one proposed in $802.11$af~\cite{TVstandard}, that enables a White-Fi network to use the white spaces. Each cell in the White-Fi network has an access point (AP) that facilitates communication between other nodes in the network and a geolocation database.}
\label{fig:80211afArch}
\end{figure}
Each cell in the White-Fi network has a geolocation database-dependent enabling (GDD-enabling~\cite{TVstandard}) access point (AP). While the AP is like any node in the cell, unlike others, it has access to the geolocation database, which keeps updated information about the TV network. The AP of every cell in the network sends the \emph{White-Fi cell map} (WCM), which consists of the locations of all nodes in the cell, to the geolocation database. The database uses the TV network information and the location information of the nodes as an input to the proposed algorithms. The resulting channel, power, and access allocations are communicated to the access points as the \emph{white space map} (WSM)~\cite{TVstandard}, which then communicate the same to nodes in their respective cells. The time granularity at which the above exchange of messages between the geolocation database and the nodes in the White-Fi cells can take place will determine limits on mobility of the nodes in the cells and the ability of the White-Fi network to adapt to changes in the TV network.


%Specifically, the access point in the White-Fi cell securely accesses the database to (a) send the White-Fi cell map (WCM) i.e. locations of Tx-Rx pairs within the cell, and (b) receive the white space map (WSM) i.e. the resultant of the proposed optimization problem which includes the operating frequencies, transmit power and access probabilities. Assuming the access point has the authority to enable and control the operation of the White-Fi nodes within the cell, the white space map is communicated to the White-Fi nodes for transmission.
%IEEE $802.11$af standard~\cite{TVstandard} specifies the requirements for spectrum sharing among unlicensed devices and TV networks in TVWS. The standard proposes the use of geolocation database, which stores, by geographic location, information about TV networks. The geolocation database can be employed to incorporate the proposed approach to provide the operating parameters for White-Fi nodes while fulfilling the regulatory requirements. 
%Figure~\ref{fig:discussion} shows an example TVWS network including the geolocation database. 
%The access point in the White-Fi cell securely accesses the database to (a) send the White-Fi cell map (WCM) i.e. locations of Tx-Rx pairs within the cell, and (b) receive the white space map (WSM) i.e. the resultant of the proposed optimization problem which includes the operating frequencies, transmit power and access probabilities. Assuming the access point has the authority to enable and control the operation of the White-Fi nodes within the cell, the white space map is communicated to the White-Fi nodes for transmission.
%\begin{itemize}
%\item The geolocation database stores, by geographic location, the permissible frequencies and provides the operating parameters for White-Fi devices to fulfill regulatory requirements.
%\item Access points securely accesses the geolocation database to (a) send the White-Fi cell map (WCM) i.e. locations of Tx-Rx pairs within its coverage and (b) obtain the White space map (WSM) i.e. the operating frequencies and parameters permitted in the White-Fi cell. We assume that the access point has the authority to enable and control the operation of the White-Fi nodes under its service.
%\item White-Fi nodes obtain the permitted operating frequencies, transmit power and access probabilities in the form of a WSM from the access point.
%\item \textbf{Flow of information:}
%\begin{itemize}
%\item Geolocation database obtains information such as operating frequencies, TV tower location, HAAT, ERP and service contour from the regulatory bodies such as FCC, Ofcom.
%\item Access point sends the White-Fi cell map (WCM) i.e. TX-RX pair locations to the geolocation database.
%\item Based on the White-Fi cell map received from the AP, geolocation database initially computes the afflicted receiver location on the service contours of TV towers and then runs the optimization to generate the White space map.
%\item The White space map is transmitted to the access point which is further communicated to the White-fi nodes.
%\end{itemize}
%\end{itemize}

==> Proof_baseline.tex <==
\section{Non-convexity of Baseline Approach}
%\setcounter{equation}{0}
As stated in Section~\ref{sec:simulation}, we compare our \textit{proposed} approach with a \textit{baseline} that allocates the same power and access probabilities to all nodes in a cell on an assigned channel. The optimization problem corresponding to the \textit{baseline} is
\begin{align}
\text{Maximize:}&\sum_{m \in \mathcal{M}} \sum_{s \in \AssignC{m}}\left[\frac{\psuccPerChannel{s} L}{\pidle \sigma +  \sum\limits_{i\in \mathcal{N}_m}\pnodesuccPerChannel{s}{i} \left(O_{\text{sec}} + \frac{O_{\text{bits}}}{\RoPerChannel{s}} + \frac{L}{\RPerChannel{s}{i}{i'}}\right) + (1 - \pidle - \psuccPerChannel{s}) \left(\frac{L_{\text{col}}}{\RoPerChannel{s}} + L_{\text{colsec}}\right)}\right],\label{eqn:obj_baseline}\\
\text{subject to:}&\sum_{m: s\in \AssignC{m}} \sum_{i\in \mathcal{N}_m} \g{i}{l} \powerPerChannel{s}{i} \le \Imaxlimit{l},\quad\forall l \in \TVRXSet{s}, \forall s \in \cup_{m=1}^M \AssignC{m},\label{eqn:constr_1_baseline}\\
& \sum_{s\in \AssignC{m}} \powerPerChannel{s}{i} \le P_T,\qquad \forall i\in\mathcal{N}_m, \forall m \in \mathcal{M},\label{eqn:constr_2_baseline}
\end{align}
where, the power assigned to each node in the cell $\powerPerChannel{s}{i} = P^{(s)}$. Since the access probability assigned to all nodes in a cell on an assigned channel is same, the probability of successful transmission and idle slot are  $\pnodesuccPerChannel{s}{i}=\accessPerChannel{s}{}(1-\accessPerChannel{s}{})^{(\mathcal{N}_m-1)}$ and $\pidle = (1-\accessPerChannel{s}{})^{\mathcal{N}_m}$, respectively. 

We solve for a simple instance of the optimization problem~(\ref{eqn:obj_baseline})-(\ref{eqn:constr_2_baseline}) where $\mathcal{M} = 1$ and $\AssignC{m} = 1$ and $\mathcal{N}_m > 1$. For ease of exposition, we consider $\TVRXSet{s} = 1$ i.e. the channel $s$ has only one afflicted receiver. The maximization problem~(\ref{eqn:obj_baseline})-(\ref{eqn:constr_2_baseline}) can be reduced to the following minimization
\begin{align}
\text{Minimize:}&\enspace\frac{1-\tau}{\tau}\frac{\sigma}{L} +\sum\limits_{\substack{i\in \mathcal{N}_m}}\left(\frac{O_{\text{sec}}}{L} + \frac{O_{\text{bits}}}{LR_{o}} + \frac{1}{R_{ii'}}\right)+\left(\frac{(1-\tau)^{(1-\mathcal{N}_m)}}{\mathcal{N}_m\tau}-\frac{1-\tau}{\mathcal{N}_m\tau}-1\right)\left(\frac{L_{\text{col}}}{LR_{o}} + \frac{L_{\text{colsec}}}{L}\right),\label{eqn:obj_baseline_simple}\\
\text{subject to:}&\sum_{i\in \mathcal{N}_m} \g{i}{l}P \le \Imaxlimit{},\label{eqn:constr_1_baseline_simple}\\
& P \le P_T,\label{eqn:constr_2_baseline_simple}
\end{align}
We now check for convexity of the optimization problem~(\ref{eqn:obj_baseline_simple})-(\ref{eqn:constr_2_baseline_simple}). 
\begin{lemma}
If f is twice differentiable, that is, its Hessian $\nabla^2 \mathit{f}$ exists at each point in \textbf{dom} f, which is open. Then f is convex if and only if \textbf{dom} f is convex and its Hessian is positive semidefinite i.e. $\nabla^2 f(x) \succeq 0$, for all $x \in \textbf{dom} f$~\cite{boyd}.\label{lem:Lemma2}
\end{lemma}
We first check for convexity of the objective function~(\ref{eqn:obj_baseline_simple}). The Hessian matrix of the objective function~(\ref{eqn:obj_baseline_simple}) is the matrix of second partial derivatives evaluated at $(\tau,P)$ given as
\begin{align}
H_{f} &=
\begin{bmatrix}
\frac{\partial^2 f}{\partial\tau^2} & \frac{\partial^2 f}{\partial\tau\partial P}\\
\frac{\partial^2 f}{\partial\tau\partial P} & \frac{\partial^2 f}{\partial P^2}
\end{bmatrix} 
\end{align}
The second partial derivatives of the objective function~(\ref{eqn:obj_baseline_simple}) are
\begin{align}
\begin{split}
\frac{\partial^2 f}{\partial\tau^2}&= \frac{2}{\tau^{3}}\frac{\sigma}{\mathcal{N}_mL} + \left(\frac{2(1-\tau)^{(1-\mathcal{N}_m)}}{\tau^{3}} + \frac{2(1-\mathcal{N}_m)(1-\tau)^{-\mathcal{N}_m}}{\tau^{2}}\right.\\
&\quad\left.-\frac{(1-\mathcal{N}_m)\mathcal{N}_m(1-\tau)^{(-\mathcal{N}_m-1)}}{\tau}-\frac{2}{\tau^3}\right)\left(\frac{L_{\text{col}}}{LR_{o}} + \frac{L_{\text{colsec}}}{L}\right)\label{eqn:partial_1}
\end{split}\\
\frac{\partial^2 f}{\partial\tau\partial P}& = \frac{(1-\tau)^{-\mathcal{N}_m}((1-\tau)^{\mathcal{N}_m}+\mathcal{N}_m\tau - 1)}{\tau^2}\left(\frac{L_{\text{col}}}{\mathcal{N}_mL}\left(\frac{-C_{min}B}{R_{o}^{2}\log 2(1+PC_{min})}\right)\right)\label{eqn:partial_2}\\
\frac{\partial^2 f}{\partial P\partial \tau}& = \frac{(1-\tau)^{-\mathcal{N}_m}((1-\tau)^{\mathcal{N}_m}+\mathcal{N}_m\tau - 1)}{\tau^2}\left(\frac{L_{\text{col}}}{\mathcal{N}_mL}\left(\frac{-C_{min}B}{R_{o}^{2}\log 2(1+PC_{min})}\right)\right)\label{eqn:partial_3}\\
\frac{\partial^2 f}{\partial P^2}&= \frac{L_{\text{col}}C_{min}B\left(\mathcal{N}_mL\log 2\left(\frac{2R_{o}C_{min}B}{\log 2(1+PC_{min})}+R_{o}^{2}C_{min}\right) \right)}{(L\mathcal{N}_mR_{o}^2\log 2(1+PC_{min}))^2}\left(\frac{1}{\tau(1-\tau)^{\mathcal{N}_m-1}}-\frac{1-\tau}{\tau}-\mathcal{N}_m\right)\nonumber\\
&+\frac{1}{\mathcal{N}_mL}\frac{\mathcal{N}_{m}O_{bits}C_{min}B(2R_{o}\log 2(1+PC_{min})+R_{o}^2\log 2C_{min})}{(R_{o}^2\log 2(1+PC_{min}))^2}\nonumber\\
&+\frac{BC_{ii'}\left(\log 2(1+PC_{ii'})\frac{2\log_{2}(1+PC_{ii'})}{(1+PC_{ii'})}C_{ii'}+\log 2\log_{2}^2(1+PC_{ii'})C_{ii'}\right)}{\mathcal{N}_mL((1+PC_{ii'})\log 2\log_2^{2}(1+PC_{ii'}))^{2}},\label{eqn:partial_4}
\end{align}
where, $C_{ii'} = \left(\frac{h_{ii'}}{BN_0 + \sum_{k\in TV_{TX}} \q{k}{} \powerTV{k}}\right)$ and $C_{min} = \min\limits_{\forall i,i' \in \mathcal{N}_m}(C_{ii'})$. 
\begin{lemma}
Let $A=\begin{pmatrix}
a & b \\ b & c
\end{pmatrix}$ be a symmetric $2\times 2$ matrix. If $D_1 = a \geq 0$ and $D_2 = ac - b^{2} \geq 0$, then $A$ is positive semidefinite~\cite{boyd}.\label{lem:Lemma_3}
\end{lemma}
Since, $D_1$ i.e.~(\ref{eqn:partial_1}) is negative for $\tau \in [0,1]$, the Hessian is not positive semidefinite (Lemma~\ref{lem:Lemma_3}). Hence, as stated in Lemma~\ref{lem:Lemma2}, the objective function in~(\ref{eqn:obj_baseline_simple}) is non-convex. Therefore, the optimization problem in~(\ref{eqn:obj_baseline_simple})-(\ref{eqn:constr_2_baseline_simple}) is one of non-convex optimization.

==> Proof_power.tex <==
\section{Non-Convexity of Solve for Power}
\label{appendix:B}
The \textit{Solve for Power} optimization problem~(\ref{eqn:solveForPower}) in its expanded form is given in~(\ref{eqn:obj_power})-(\ref{eqn:constr3}).
\begin{table*}
\small
\vspace{-1em}
\begin{align}
\text{Maximize:}&\sum_{m \in \mathcal{M}} \sum_{s \in \AssignC{m}}\left[\frac{\psuccPerChannel{s} L}{\pidle \sigma +  \sum\limits_{i\in \mathcal{N}_m}\pnodesuccPerChannel{s}{i} \left(O_{\text{sec}} + \frac{O_{\text{bits}}}{\RoPerChannel{s}} + \frac{L}{\RPerChannel{s}{i}{i'}}\right) + (1 - \pidle - \psuccPerChannel{s}) \left(\frac{L_{\text{col}}}{\RoPerChannel{s}} + L_{\text{colsec}}\right)}\right],\label{eqn:obj_power}\\
\text{subject to:}&\sum_{m: s\in \AssignC{m}} \sum_{i\in \mathcal{N}_m} \g{i}{l} \powerPerChannel{s}{i} \le \Imaxlimit{l},\quad\forall l \in \TVRXSet{s}, \forall s \in \cup_{m=1}^M \AssignC{m},\label{eqn:constr1}\\
& \sum_{s\in \AssignC{m}} \powerPerChannel{s}{i} \le P_T,\qquad \forall i\in\mathcal{N}_m, \forall m \in \mathcal{M},\label{eqn:constr2}\\
&\frac{(1 - \accessPerChannel{s}{i})}{\accessPerChannel{s}{i}} \RPerChannel{s}{i}{i'} = \frac{(1 - \accessPerChannel{s}{j})}{\accessPerChannel{s}{j}} \RPerChannel{s}{j}{j'},\qquad \forall i,i',j,j'\in \mathcal{N}_m, \forall s\in \AssignC{m}, \forall m\in \mathcal{M}.\label{eqn:constr3}
\end{align}
\vspace{-1em}
\end{table*}
This optimization problem is non-convex in $\mathbf{P}$. The non-convexity is due to the non-linear equality constraint~(\ref{eqn:constr3}).

Also, the problem is difficult to solve and may not have an easy closed-form analytical solution. We illustrate the complexity of the \textit{Solve for Power} optimization problem by using instances of the problem in~(\ref{eqn:obj_power})-(\ref{eqn:constr3}). We begin with the simplest instance where each cell has a single link and multiple channels. The throughput maximization problem for this instance is equivalent to \textit{water-filling} and has an analytical solution.

Next, we take a step closer to the optimization problem in~(\ref{eqn:obj_power})-(\ref{eqn:constr3}) by considering the throughput maximization of a single cell with multiple links and a single channel assigned to it. The problem as we see later is non-convex in $\mathbf{P}$ due to the non-linear time fairness constraint~(\ref{eqn:constr3}). Further, an analytical solution to the optimization problem using the Lagrangian method is infeasible. Next, we describe the two problems in detail.
\subsection{Single link, multiple channels and single cells ($\mathcal{N}_m = 1,\AssignC{m}>1, \mathcal{M} = 1$)} Consider a network comprising of a cell with a single link and multiple channels. On any channel $s$, the probability of medium access of the link  i.e. $\accessPerChannel{s}{} = 1$. Therefore, the probability of successful transmission, $\psuccPerChannel{s} = 1$, probability of an idle slot $\pidle = 0$. We assume no overhead bits i.e. $O_{bits} = 0$ and $O_{sec} = 0$. The resulting optimization problem is
\begin{align}
\text{Maximize:}&\nonumber\\
&\hspace{-4.5em}\sum_{m \in \mathcal{M}}\sum_{s\in \AssignC{m}}B\log_2\left(1 + \frac{\hPerChannel{s}{}{} \powerPerChannel{s}{}}{BN_0 + \sum_{k\in \TVTXSet{s}} \q{k}{} \powerTV{k}}\right),\label{eqn:waterfilling_obj}\\
%\sum_{s\in \AssignC{}}
\text{subject to:}&\ \g{}{l} \powerPerChannel{s}{} \le \Imaxlimit{l},\enspace\forall l \in \TVRXSet{s}, \forall s \in \AssignC{m},\label{eqn:waterfilling_const_1}\\
& \sum_{s\in \AssignC{m}} \powerPerChannel{s}{} \le P_T,\quad \forall m\in \mathcal{M}.\label{eqn:waterfilling_const_2}
\end{align}
The optimization problem is akin to a \textit{water-filling} problem~\cite[Chapter~5]{boyd}. The objective function in~(\ref{eqn:waterfilling_obj}) is jointly concave in the powers and the optimization problem can be solved by Lagrangian methods. For ease of exposition, we consider $\TVRXSet{s} = 1$ i.e. each channel $s \in \AssignC{m}$ has one afflicted receiver. Consider the Lagrangian
\begin{align}
\mathcal{L}(\mathbf{P},\bm{\mu}) &= \sum_{s\in\AssignC{m}}B\log_2\left(1 + \frac{\hPerChannel{s}{}{} \powerPerChannel{s}{}}{BN_0 + \sum_{k\in \TVTXSet{s}} \q{k}{} \powerTV{k}}\right)\nonumber\\ 
&\qquad-\sum\limits_{s\in\AssignC{m}}\mu_{s} (\g{}{l} \powerPerChannel{s}{} - \Imaxlimit{l})\nonumber\\
&\qquad\qquad-\mu_{\AssignC{m}+1}\left(\sum\limits_{s\in \AssignC{m}}\powerPerChannel{s}{} - P_T\right),
\end{align}
where, $\bm{\mu} =\{\mu_{1},\dots,\mu_{\AssignC{m}+1}\}$ are the KKT multipliers. The Kuhn-Tucker condition are:
\begin{align}
&\mu_{1},\dots,\mu_{\AssignC{m}+1} \geq 0, \label{eqn:KKT_waterfilling_1}\\
&\frac{\partial \mathcal{L}}{\partial \powerPerChannel{s}{}} = 0,\quad \forall s\in \AssignC{m},\label{eqn:KKT_waterfilling_2}\\
&\mu_{s} (\g{}{l} \powerPerChannel{s}{} - \Imaxlimit{l}) = 0,\quad \forall l \in \TVRXSet{s}, \forall s\in \AssignC{m},\label{eqn:KKT_waterfilling_3}\\
&\mu_{\AssignC{m}+1} \left(\sum\limits_{s\in\AssignC{m}}\powerPerChannel{s}{} - P_T\right) = 0,\label{eqn:KKT_waterfilling_4}\\
&\g{}{l} \powerPerChannel{s}{} \le \Imaxlimit{l},\quad \forall l \in \TVRXSet{s},\forall s \in \AssignC{m},\label{eqn:KKT_waterfilling_5}\\
&\sum_{s\in \AssignC{m}} \powerPerChannel{s}{} \le P_T.\label{eqn:KKT_waterfilling_6}
\end{align}
On solving~(\ref{eqn:KKT_waterfilling_1})-(\ref{eqn:KKT_waterfilling_6}), we get the optimal power allocation, $\forall s\in \AssignC{m}$,
\begin{align}
{\powerPerChannel{s}{}}^{*}& = \left(\frac{1}{\mu_{s}\g{}{l} + \mu_{\AssignC{m}+1}} - \frac{BN_0 + \sum_{k\in \TVTXSet{s}} \q{k}{} \powerTV{k}}{\hPerChannel{s}{}{}}\right).
\end{align}
This power allocation is optimal, with the KKT multipliers {\boldmath$\mu$} chosen such that the constraints in~(\ref{eqn:waterfilling_const_1}) and~(\ref{eqn:waterfilling_const_2}) are met.

\subsection{Multiple links, single channel and single cell ($\mathcal{N}_m > 1,\AssignC{m} = 1, \mathcal{M} = 1$)} The throughput maximization for a network with a single cell comprising of multiple links and a single channel assigned to it is 
\begin{align}
\text{Maximize:}&\ %\sum_{m\in \mathcal{M}}\sum_{s\in \AssignC{m}}
\frac{p_{\text{succ}} L}{\sigmaAvg},\label{eqn:obj_power_instance2}\\
%\frac{p_{\text{succ}} L}{p_{\text{idle}} \sigma +  \sum\limits_{i\in \mathcal{N}_m}p_{\text{succ,i}} \left(O_{\text{sec}} + \frac{O_{\text{bits}}}{R_{o}} + \frac{L}{R_{ii'}}\right) + (1 - p_{\text{idle}} - p_{\text{succ}}) \left(\frac{L_{\text{col}}}{R_{o}} + L_{\text{colsec}}\right)},\label{eqn:obj_power_instance2}\\
\text{subject to:}&\sum_{i\in \mathcal{N}_m} \g{i}{l} P_{i} \le \Imaxlimit{}, \label{eqn:constr1_instance2}\\
& P_{i} \le P_T,\qquad \forall i\in\mathcal{N}_m,\label{eqn:constr2_instance2}\\
&\frac{(1 - \tau_{i})}{\tau_{i}} \R{ii'} = \frac{(1 - \tau_{j})}{\tau_{j}} \R{jj'},\enspace\forall i,i',j,j'\in \mathcal{N}_m,\label{eqn:constr3_instance2}
\end{align}

where, $\sigmaAvg$ for single channel can be obtained from~(\ref{eqn:avgSlot}). For ease of exposition, we assume that the channel assigned to the cell has only one afflicted receiver. The maximization problem in~(\ref{eqn:obj_power_instance2})-(\ref{eqn:constr3_instance2}) can be reduced to the following minimization
\begin{align}
&\text{Minimize:}\smallskip\frac{1}{R_{o}}\left(f_{3}(\tau) + \sum\limits_{\substack{i\in \mathcal{N}_m}}f_{2}^{(i)}(\tau)O_{\text{bits}}\right)+\sum\limits_{\substack{i\in \mathcal{N}_m}}\frac{f_{2}^{(i)}L}{R_{ii'}}\label{eqn:obj_power_instance2a}\\
&\text{subject to:}\smallskip(\ref{eqn:constr1_instance2}), (\ref{eqn:constr2_instance2}), (\ref{eqn:constr3_instance2}),\label{eqn:constr_power_instance2a}
\end{align}
where, $f_{2}^{(i)}(\tau) = \frac{p_{\text{succ,i}}}{p_{\text{succ}}L}$ and $f_{3}(\tau) = \left(\frac{1}{p_{\text{succ}}}-\frac{p_{\text{idle}}}{p_{\text{succ}}}-1\right)\frac{L_{\text{col}}}{L}$, respectively. The objective function ~(\ref{eqn:obj_power_instance2a}) is jointly convex in the powers, however, due to the non-linear equality constraint~(\ref{eqn:constr3_instance2}) the optimization problem is non-convex in $\mathbf{P}$. The Lagrangian of the optimization problem~(\ref{eqn:obj_power_instance2a})-(\ref{eqn:constr_power_instance2a}) is
\begin{align}
\mathcal{L}(\mathbf{P},\bm{\mu},\bm{\lambda}) &= \frac{1}{R_{o}}\left(f_{3}(\tau) + \sum\limits_{\substack{i\in \mathcal{N}_m}}f_{2}^{(i)}(\tau)O_{\text{bits}}\right)\nonumber\\
&\quad+\sum\limits_{\substack{i\in \mathcal{N}_m}}\frac{f_{2}^{(i)}L}{R_{ii'}} +  \sum\limits_{i\in \mathcal{N}_m} \mu_{i}\left(P_{i} - P_T\right)\nonumber\\ 
&\qquad+\mu_{\mathcal{N}_m+1}\left(\left(\sum_{i\in \mathcal{N}_m} \g{i}{l} P_{i}\right) - \Imaxlimit{}\right)\nonumber\\
&\qquad\quad+\sum\limits_{k\in \mathcal{N}_m} \lambda_{k}\left(\frac{1 - \tau_{i}}{\tau_{i}} R_{ii'} - \frac{1 - \tau_{j}}{\tau_{j}} R_{jj'}\right)
\end{align}
where, $\bm{\mu} = \{\mu_1,\dots,\mu_{\mathcal{N}_m+1}\}$ is the KKT multiplier vector and $\bm{\lambda} = \{\lambda_1,\dots,\lambda_{\mathcal{N}_m}\}$ is the Lagrangian multiplier vector. The KKT conditions for the optimization problem~(\ref{eqn:obj_power_instance2a})-(\ref{eqn:constr_power_instance2a}) are
\begin{align}
&\mu_1,\dots,\mu_{\mathcal{N}_m+1} \geq 0,\\
&\frac{\partial \mathcal{L}}{\partial P_{i}} = 0,\quad \forall i\in \mathcal{N}_m,\\
& \mu_{i} \left(P_{i}-P_T\right) = 0,\qquad \forall i\in\mathcal{N}_m,\\
&\mu_{\mathcal{N}_m+1}\left(\left(\sum_{i\in \mathcal{N}_m} \g{i}{l} P_{i}\right) - \Imaxlimit{}\right) = 0,\\
& P_{i} \leq P_T,\qquad \forall i\in\mathcal{N}_m,\\
&\sum_{i\in \mathcal{N}_m} \g{i}{l} P_{i} \leq \Imaxlimit{},\\
&\frac{(1 - \tau_{i})}{\tau_{i}} R_{ii'} = \frac{(1 - \tau_{j})}{\tau_{j}} R_{jj'},\enspace\forall i,i',j,j'\in \mathcal{N}_m.
\end{align}
Note that this simple instance requires us to solve $(5\mathcal{N}_m + 3)$ KKT conditions, few of which are non-linear, making the solution to the optimization problem intractable. Adding multiple cells with multiple links per cell and multiple channels assigned further increases the complexity. Hence, indicating the difficulty of the  problem~(\ref{eqn:obj_power})-(\ref{eqn:constr3}) and intractability of an analytical solution for the same.

==> Proof_tau_old.tex <==
\section{Convexity of Solve for Access}
\label{appendix:A}
The \textit{Solve for Access} optimization problem that solves for a vector of access probabilities $\mathbf{\Psi}$ that maximizes the White-Fi network throughput $T$ defined in~(\ref{eqn:netwkThr}), for a given transmit power vector $\mathbf{P}^*$ is
\begin{align*}
\text{Maximize:}&\ T(\mathbf{\Psi},\mathbf{P}^*),\quad {\text{subject to:}}\ (\ref{eqn:fairness}).
\end{align*}
Since the power vector is given, the optimization problem can be separated into maximizing throughputs $\throughputCellCh{m}{s}$ for each selection of cell $m$ and channel $s$, where $s$ is a channel in the set of channels assigned to $m$. For every such selection of $m$ and $s$, we must choose access probabilities $\accessPerChannel{s}{j}$, for every node $j$ in cell $m$, such that $\throughputCellCh{m}{s}$ is maximized. The throughput maximization problem can be reduced to a minimization problem in single-variable, $\accessPerChannel{s}{j}$ of certain node $j$ in the cell, using the time fairness constraint~(\ref{eqn:fairness}) (detailed next). We assume that node $j$ corresponds to the node with the minimum payload rate.

The throughput of the $i^{th}$ node in cell $m$ on a channel $s$ assigned to it is given as
\begin{align}
\throughputCellCh{i,m}{s} =  \frac{\pnodesuccPerChannel{s}{i} L}{\pidle \sigma +  \sum_{i\in \mathcal{N}_m}\pnodesuccPerChannel{s}{i} \Tnodesucc{i} + (1 - \pidle - \psuccPerChannel{s}) \Tcol}.
\label{eqn:perCellPerChannelPerNodeTh}
\end{align}
%where,
%\begin{align*}
%\pnodesuccPerChannel{s}{i} & = \accessPerChannel{s}{i}\prod\limits_{\substack{j\in \mathcal{N}_m \\ j\neq i}}(1-\accessPerChannel{s}{j}),\quad
%\psuccPerChannel{s} = \sum_{i\in\mathcal{N}_m} \pnodesuccPerChannel{s}{i},\quad
%\pidle = \prod\limits_{i\in \mathcal{N}_m}(1-\accessPerChannel{s}{i}),\quad
%\pcolPerChannel{s} = (1 - \pidle - \psuccPerChannel{s}),\\
%\Tnodesucc{i} & = (O_{\text{sec}} + O_{\text{bits}}/\RoPerChannel{s} + L/\RPerChannel{s}{i}{i'}),\quad
%\Tcol = (L_{\text{col}}/\RoPerChannel{s} + L_{\text{colsec}}).
%\end{align*}
On simplifying~(\ref{eqn:perCellPerChannelPerNodeTh}) we get
\begin{align}
\throughputCellCh{i,m}{s} = \left[\frac{1}{L}\left(\frac{\pidle}{\pnodesuccPerChannel{s}{i}}\sigma +\Tnodesucc{i} + \left(\sum\limits_{\substack{j\in \mathcal{N}_m \\ j\neq i}}\frac{\pnodesuccPerChannel{s}{j}}{\pnodesuccPerChannel{s}{i}}\Tnodesucc{j}\right)+\left(\frac{1}{\pnodesuccPerChannel{s}{i}}-\frac{\pidle}{\pnodesuccPerChannel{s}{i}}-1-\sum\limits_{\substack{j\in \mathcal{N}_m \\ j\neq i}}\frac{\pnodesuccPerChannel{s}{j}}{\pnodesuccPerChannel{s}{i}}\right)\Tcol\right)\right]^{-1}.
\end{align}
The probability $\pnodesuccPerChannel{s}{i}$ that a transmission by $i$ is successful and the probability $\pidle$ that a slot is idle is given in~(\ref{eqn:psuccAndIdleForANode}). According to time fairness constraint~(\ref{eqn:fairness}), 
$\pnodesuccPerChannel{s}{i}\RPerChannel{s}{j}{j'} = \pnodesuccPerChannel{s}{j}\RPerChannel{s}{i}{i'}$, which can be  simplified to
\begin{align}
\frac{(1 - \accessPerChannel{s}{i})}{\accessPerChannel{s}{i}} \RPerChannel{s}{i}{i'} &= \frac{(1 - \accessPerChannel{s}{j})}{\accessPerChannel{s}{j}} \RPerChannel{s}{j}{j'},\quad \forall i,i',j,j'\in \mathcal{N}_m, \forall s\in \AssignC{m}, \forall m\in \mathcal{M}.
\end{align}
By substituting $\pnodesuccPerChannel{s}{i}$ and $\pidle$ from~(\ref{eqn:psuccAndIdleForANode}) and using the time fairness constraint~(\ref{eqn:fairness}) we get
\begin{align}
\throughputCellCh{i,m}{s} &= \left[f_{1}(P) + \frac{\RPerChannel{s}{j}{j'}}{L\RPerChannel{s}{i}{i'}} \left(\frac{1-\accessPerChannel{s}{j}}{\accessPerChannel{s}{j}}\sigma+\left(\frac{1}{\accessPerChannel{s}{j}\prod\limits_{\substack{j\in \mathcal{N}_m \\ j\neq k}}(1-\accessPerChannel{s}{k})}-\frac{1-\accessPerChannel{s}{j}}{\accessPerChannel{s}{j}}-f_{2}(P)\right)\Tcol\right)\right]^{-1},\nonumber\\
&= \left[f_{1}(P) + \frac{\RPerChannel{s}{j}{j'}}{L\RPerChannel{s}{i}{i'}} \left(\frac{1-\accessPerChannel{s}{j}}{\accessPerChannel{s}{j}}\sigma+\left(\prod\limits_{k\in \mathcal{N}_m }\left(\frac{\RPerChannel{s}{k}{k'}}{\RPerChannel{s}{j}{j'}} +\frac{1-\accessPerChannel{s}{j}}{\accessPerChannel{s}{j}}\right)-\frac{1-\accessPerChannel{s}{j}}{\accessPerChannel{s}{j}}-f_{2}(P)\right)\Tcol\right)\right]^{-1},\nonumber\\
&\text{where}\ f_{1}(P) = \frac{\Tnodesucc{i}}{L} + \left(\sum\limits_{\substack{j\in \mathcal{N}_m \\ j\neq i}}\frac{\RPerChannel{s}{j}{j'}}{L\RPerChannel{s}{i}{i'}}\Tnodesucc{j}\right),\enspace f_{2}(P) = \frac{\RPerChannel{s}{i}{i'}}{\RPerChannel{s}{j}{j'}}\left(1+\sum\limits_{\substack{j\in \mathcal{N}_m \\ j\neq i}}\frac{\RPerChannel{s}{j}{j'}}{\RPerChannel{s}{i}{i'}}\right).\nonumber
\end{align}
The throughput maximization problem can be reduced to the following minimization
\begin{align}
&\text{Minimize:} \left(\frac{1-\accessPerChannel{s}{j}}{\accessPerChannel{s}{j}}\sigma+\left(\prod\limits_{k\in \mathcal{N}_m }\left(\frac{\RPerChannel{s}{k}{k'}}{\RPerChannel{s}{j}{j'}} +\frac{1-\accessPerChannel{s}{j}}{\accessPerChannel{s}{j}}\right)-\frac{1-\accessPerChannel{s}{j}}{\accessPerChannel{s}{j}}-f_{2}(P)\right)\Tcol\right)\nonumber ,\\
&{\text{subject to:}}\enspace 0 \leq\accessPerChannel{s}{j}\leq 1.
\label{eqn:min}
\end{align}
We now show that the minimization problem~(\ref{eqn:min}) is a convex optimization problem. The objective function $f(\accessPerChannel{s}{j})$ is
\begin{align}
& f(\accessPerChannel{s}{j}) = f_{1}(\accessPerChannel{s}{j})\sigma+f_2(\accessPerChannel{s}{j})\Tcol\nonumber\\
&\text{where}\ f_{1}(\accessPerChannel{s}{j}) = \frac{1-\accessPerChannel{s}{j}}{\accessPerChannel{s}{j}},\enspace f_{2}(\accessPerChannel{s}{j}) = \prod\limits_{k\in \mathcal{N}_m }\left(\frac{\RPerChannel{s}{k}{k'}}{\RPerChannel{s}{j}{j'}} +\frac{1-\accessPerChannel{s}{j}}{\accessPerChannel{s}{j}}\right)-\frac{1-\accessPerChannel{s}{j}}{\accessPerChannel{s}{j}} -f_{2}(P)
\label{eqn:funcTau}
\end{align}
$f_{1}(\accessPerChannel{s}{j})$ is a non-increasing convex function on the interval $[0,1]$. Next, we show that the function $f_{2}(\accessPerChannel{s}{j})$ is also a convex function.
\begin{align}
f_{2}(\accessPerChannel{s}{j}) & = \prod\limits_{k\in \mathcal{N}_m }\left(\frac{\RPerChannel{s}{k}{k'}}{\RPerChannel{s}{j}{j'}} +\frac{1-\accessPerChannel{s}{j}}{\accessPerChannel{s}{j}}\right)-\frac{1-\accessPerChannel{s}{j}}{\accessPerChannel{s}{j}} -f_{2}(P)\nonumber\\
& = \frac{1}{\accessPerChannel{s}{j}}\left(\prod\limits_{\substack{k\in \mathcal{N}_m \\ k\neq j}} \left(\frac{\RPerChannel{s}{k}{k'}}{\RPerChannel{s}{j}{j'}} +\frac{1-\accessPerChannel{s}{j}}{\accessPerChannel{s}{j}}\right)-1\right)+1-f_{2}(P)
\end{align}
\begin{lemma}
If $f:\mathcal{R}\rightarrow \mathcal{R}:x\mapsto f(x)$ and $g:\mathcal{R}\rightarrow \mathcal{R}:x\mapsto g(x)$ are both convex, non-decreasing (or non-increasing) and positive, then $h:\mathcal{R}\rightarrow \mathcal{R}:x\mapsto h(x) = f(x)g(x)$ is also convex~\cite{boyd}.\label{lem:Lemma1}
\end{lemma}
We see that $f_{2}(\accessPerChannel{s}{j})$ consists of a product of $\frac{1}{\accessPerChannel{s}{j}}$ and $\left(\prod\limits_{\substack{k\in \mathcal{N}_m \\ k\neq j}} \left(\frac{\RPerChannel{s}{k}{k'}}{\RPerChannel{s}{j}{j'}} +\frac{1-\accessPerChannel{s}{j}}{\accessPerChannel{s}{j}}\right)-1\right)$. Both the functions are convex, non-increasing and positive function on the interval $[0,1]$. Hence, using Lemma~\ref{lem:Lemma1}, the product of these functions i.e. $f_{2}(\accessPerChannel{s}{j})$ is also convex on the interval $[0,1]$.

Therefore, $f(\accessPerChannel{s}{j})$ in~(\ref{eqn:min}) is a non-negative weighted sum of convex functions i.e. $f_{1}(\accessPerChannel{s}{j})$ and $f_{2}(\accessPerChannel{s}{j})$, and hence a convex function~\cite{boyd}. As a result, the optimization problem in~(\ref{eqn:min}), minimizes a convex function over a convex set and is therefore, a convex optimization problem.

==> abstract.tex <==
\begin{abstract}
White-Fi refers to WiFi deployed in the TV white spaces. Unlike its ISM band counterparts, White-Fi must obey requirements that protect TV reception. As a result, optimization of citywide White-Fi networks faces the challenges of heterogeneous channel availability and signal quality, over location. (a) The former is because, at any location, channels in use by TV networks are not available for use by White-Fi. (b) The latter is because the signal quality available at a White-Fi receiver is determined by not only its link gain to its transmitter but also by its link gains to primary transmitters and its transmitter's link gains to primary receivers.

In this work, we model the medium access control (MAC) throughput of a White-Fi network. We propose heuristic algorithms to optimize the throughput, given the described heterogeneity. The algorithms assign power, access probability, and channels to nodes in the network, under the constraint that signal quality at TV receivers is not compromised. We evaluate the efficacy of our approach over example city-wide White-Fi networks deployed over Denver and Columbus (respectively, low and high channel availability) in the USA, and compare with assignments cognizant of heterogeneity to a lesser degree, for example, based on FCC regulations.
\end{abstract}
%TV white spaces (TVWS) are the unused frequencies in the VHF/UHF band. IEEE $802.11$af, also known as White-Fi and Super-WiFi standard, allows WiFi like networks to be deployed in TVWS. However, unlike the unlicensed bands ($2.4$ and $5$ GHz), where Wi-Fi networks are commonly deployed, TVWS see significant variation in channel availability and quality over space. This spatial variation can be credited to TV networks operating in the vicinity of the White-Fi network. Also, White-Fi cells can have coverage as large as $5$ kms, resulting in nodes seeing large variation in channel quality. This motivates our investigation into the optimization of a White-Fi network that spans a large area and therefore constitutes multiple cells. The optimization problem is to assign TVWS channels, transmit power and channel access probabilities to nodes in a city-wide White-Fi network such that the saturated WiFi throughput is maximized under the constraint that the aggregate interference at the TV receivers is within acceptable limits. The problem is non-convex. We solve it heuristically and present evaluation of our approach over the example cities of Denver (low channel availability) and Columbus (high channel availability) in the US.


==> capacity.tex <==
%\section{Network Throughput}
%\label{sec:capacity}
%\begin{figure}
%\begin{center}
%\includegraphics[width=0.5\columnwidth]{Figures/Simulation_Setup_sg.pdf}
%\caption{\small Example White-Fi cell with a total of $20$ nodes. Nodes $i$ and $i'$ transmit unicast packets to each other. TV network consists of a transmitter (large tower) and a receiver. Example gains $\hPerChannel{c}{i}{j}$ between nodes $i=1'$ and $j=3$ in the White-Fi cell, gains $\gPerChannel{c}{i}{l}$ from a node $i=3'$ in the White-Fi cell to the TV receiver, and gains from the TV transmitter to node $3'$, are shown over channel $c=21$.}
%\label{fig:simulationTopology}%
%\end{center}
%\vspace{-0.1in}
%\end{figure}
%Consider $\mathcal{\overline{C}}_m \subset \mathcal{C}_m$ denote the set of channels assigned to any cell $m$. We will first elucidate the various aspects of the model for a single White-Fi cell assigned any channel $c \in \mathcal{\overline{C}}_m$ and then extend the formulation to $M$ White-Fi cells. 
%%and then state the optimization problem for one or more assigned channels. 
%Let $\mathcal{N} = \{1,2,\ldots,N\}$ denote the set of nodes in the White-Fi cell. The nodes can transmit over one or more white space channels. Let $B$ denote the channel bandwidth. Node $i\in \mathcal{N}$ transmits unicast packets with power $\power{i}$. Let $\h{i}{j}$ be the link gain between nodes $i,j\in\mathcal{N}$.
%Let the White-Fi cell $m$, coexist with $K$ primary networks indexed $\{1,2,\ldots,K\}$. Let $\powerTV{k}$ be the transmit power of the TV transmitter of primary network $k$. Let $\q{k}{i}$ be the channel gain between TV transmitter of primary network $k$ and the White-Fi node $i$. Let $N_0$ be the power spectral density of additive white Gaussian (AWGN) noise at a White-Fi node. The rate $\R{i}{j}$ that can be achieved when node $i$ transmits to node $j$ is given by the Shannon's rate formula 
%\begin{align}
%&\R{i}{j} = B\log_2(1 + \SINR{i}{j})\ \text{bits/sec},\label{eqn:wifiLinkRate}\\
%&\text{where}\ \SINR{i}{j} = \frac{\h{i}{j} \power{i}}{BN_0 + \sum_{k=1}^K \q{k}{i} \powerTV{k}}.\label{eqn:wifiLinkSINR}
%\end{align}
%Note that while the channel gains between the White-Fi nodes are symmetric, that is $\h{i}{j} = \h{j}{i}$, the rates on the forward and reverse links are unlikely to be equal. That is $\R{i}{j} \ne \R{j}{i}$. This is because, for a White-Fi cell with a large spatial span, $\sum_{k=1}^K \q{k}{i} \powerTV{k} \ne \sum_{k=1}^K \q{k}{j} \powerTV{k}$, and as we will see later in Section~\ref{sec:results}, $\power{i} \ne \power{j}$.
%
%All White-Fi nodes follow the IEEE $802.11$ distributed coordination function (DCF) to access the wireless medium. The DCF~\cite{bianchi} is a CSMA/CA (Carrier Sense Multiple Access/ Collision Avoidance) based random access scheme. We will consider a White-Fi cell in which all nodes can decode control messages like request-to-send (RTS), clear-to-send (CTS), ACK, sent from any other node in the cell. So while the data packet sent by $i$ to $j$ at rate $\R{i}{j}$ may not be correctly decoded by another node $n$, all control messages sent by $i$ must be correctly decoded by $n$. Note that the overheads transmitted by node $i$ can be correctly decoded by any other node in the cell if they are sent at a rate not greater than $B \log_2(1 + \min_{j\in \mathcal{N}, j\ne i} \SINR{i}{j})$. In this work we will assume that all nodes within a cell $m$, use the same rate $\Ro$ to send overheads, which is given by
%\begin{align}
%\Ro = \min_{i\in\mathcal{N}} B \log_2(1 + \min_{\substack{j\ne i\\j\in\mathcal{N}}} \SINR{i}{j}).\label{eqn:overheadRate}
%\end{align}
% 
%A DCF slot during which no transmission takes place is an idle slot. A slot in which exactly one node transmits sees a successful transmission. A slot in which more than one node transmits sees a collision and none of the transmitted packets are decoded successfully. Let $\access{i}$ be the steady state probability with which White-Fi node $i$ accesses the wireless medium in a DCF slot. The probability $\pnodesucc{i}$ that a transmission by $i$ is successful and the probability $p_{\text{idle}}$ that a slot is idle are
%\begin{align}
%\pnodesucc{i} = \access{i}\prod\limits_{\substack{k=1 \\ k\neq i}}^{N}(1-\access{k}),\ \text{and } \pidle = \prod_{i=1}^{N}(1-\access{i}).
%\label{eqn:psuccAndIdleForANode}
%\end{align}
%Let idle slots be of duration $\sigma$. Let $L$ bits be the size of payload in a packet transmitted by any White-Fi node $i$. A slot that sees a successful transmission consists of the payload, overhead bits including packet headers, RTS/CTS, ACK, and overheads due to inter frame spacings like DIFS. Let $O_{\text{bits}}$ be the number of overhead bits. They are transmitted at the overhead rate $\Ro$. The payload is transmitted by node $i$ to its destination node, say $i'$, at rate $\R{i}{i'}$. Let $O_{\text{sec}}$ denote the frame spacing related overheads. Therefore, the total duration of a successful transmission slot of node $i$ is given by $\Tnodesucc{i} = O_{\text{sec}} + O_{\text{bits}}/\Ro + L/\R{i}{i'}$.
%
%Finally, a slot that sees a collision has $L_{\text{col}}$ bits and $L_{\text{colsec}}$ time overheads. The duration of a collision is given by $\Tcol = L_{\text{col}}/\Ro + L_{\text{colsec}}$. On use of RTS/CTS, which we assume in this work\footnote{The case when the network does not use RTS/CTS introduces variable length collisions, where the length is a function of the payload rates of the colliding transmissions. While, this can be incorporated in the model, the resulting expression for the length of the collision slot becomes unwieldy. Also, as is shown in~\cite{bianchi}, under saturation conditions the maximum throughput with or without RTS/CTS is the same. In fact, using RTS/CTS is more desirable as it makes the throughput less sensitive to small changes in access probability.}, only RTS packets may collide. As a result, $\Tcol$ is the same irrespective of which nodes' transmissions were involved in a collision. Following the analysis in~\cite{bianchi}, we can now calculate the length $\sigmaAvg$ of an average DCF slot as
%\begin{align}
%\sigmaAvg = \pidle \sigma +  \sum_{i\in \mathcal{N}}\pnodesucc{i} \Tnodesucc{i} + (1 - \pidle - \psucc) \Tcol,
%\label{eqn:avgSlot}
%\end{align}
%where $\psucc = \sum_{i\in\mathcal{N}} \pnodesucc{i}$.
%
%Note that all quantities in equations~(\ref{eqn:wifiLinkRate})-(\ref{eqn:avgSlot}) are defined and calculated for any assigned channel. When referring to a quantity for a specific assigned channel $c$ we will use the superscript $^{(c)}$. So the probability of successful transmission in channel $c$ is denoted as $\pnodesuccPerChannel{c}{i}$. This probability was first defined for node $i$ for any assigned channel in equation~(\ref{eqn:psuccAndIdleForANode}). Similarly, the power that a node $i$ puts into a channel $c$ is given by $\powerPerChannel{c}{i}$. 
%
%We will assume that all nodes always have a packet to send. For any cell $m$, the saturation throughput $\throughputSub{c}$ in any assigned channel $c$ and the sum-throughput calculated over the set of assigned channels $\mathcal{\overline{C}}_m$, are given by
%\begin{align}
%\throughputSub{c} =  \frac{\psuccPerChannel{c} L}{\sigmaAvgPerChannel{c}}\ \text{and } \throughputCell{m} = \sum_{c=1}^{|\mathcal{\overline{C}}_{m}|} \throughputSub{c}.\label{eqn:throughput}
%\end{align}
%
%The assumption that all nodes within a cell can hear control overheads like RTS/CTS sent by others in the cell allows us to use the analysis in~\cite{bianchi} to arrive at the saturation throughput of a White-Fi cell in equation~(\ref{eqn:throughput}). However, it precludes the possibility of hidden nodes in the network. There are many works that extend~\cite{bianchi} to model the throughput in the presence of hidden nodes. It is noteworthy that the extension in~\cite{ekici_ieee_2008} uses the same basic form of throughput as in~\cite{bianchi} and is amenable to per node payload rates and access probabilities, and optimizable overhead rates. That said, the extension to hidden nodes is non-trivial and we defer it to the future. Among other things, not all nodes in the cell see the same set or number of hidden nodes. Lastly, the basic interplay between the White-Fi network and the primary, which involves interference created by TV transmitters at White-Fi nodes and the interference created by the nodes at TV receivers, is captured well by the White-Fi network under consideration.
%
%The network throughput calculated over the cells indexed $1,2,\ldots,M$ is given by
%\begin{align}
%\throughput = \sum_{m=1}^{M} \throughputCell{m}.\label{eqn:throughputnet}
%\end{align}
%Figure~\ref{fig:simulationTopology} shows a White-Fi cell flanked by a primary network operating on channel $21$.

